From Parameters to Feature Space: Task Arithmetic for Backdoor Mitigation in Model Merging

Model merging (MM) has gained significant attention as a cost-effective approach to integrate multiple task-specific models into a unified model. However, recent work reveals that MM is highly susceptible to backdoor attacks. Existing defenses based on task arithmetic often fail to eliminate backdoors without substantially degrading clean-task performance, owing to their reliance on direct parameter-space editing. To address this gap, we propose Linear Feature Path Minimization (LFPM), a backdoor mitigation framework for model merging, which introduces an anti-backdoor task vector into the backdoored merged model. Unlike prior approaches, LFPM formulates the backdoor robustness of the merged model from a unified feature-space perspective under the Cross-Task Linearity (CTL) framework, which leverages the approximate linearity of features across tasks. This perspective guides the optimization of the anti-backdoor task to suppress backdoors while preserving clean-task performance. Furthermore, we introduce an effective optimization mechanism based on gradient accumulation and loss path-integral, ensuring robust backdoor suppression along the interpolation path. Extensive experiments demonstrate that LFPM consistently exhibits strong robustness against backdoor attacks in both full fine-tuning and Parameter-Efficient Fine-Tuning (PEFT) settings.

==> section/implementation_details/curvature_analysis.tex <==
% \textbf{Motivation.} To better understand the underlying principles of LFPM and empirically validate the Cross-Task Linearity (CTL) condition, we perform a 
% curvature analysis along the parameter interpolation path. As discussed in Section~\ref{section:stability_factors_for_ctl}, the CTL condition is controlled by 
% the deviation
% \begin{equation}
% \mathcal{C}(\theta; \delta) = \left \| \delta^{\top} H(\theta(t)) \delta \right \|
% \label{eq:curvature_def_appendix}
% \end{equation}
% where $H(\theta) = \nabla^2 f(\theta(t))$ denotes the Hessian matrix of the network, and $\delta = \theta_j - \theta_i$ represents the difference between the endpoint 
% models along the interpolation path.

% This measure quantity measures the deviation between the features produced by the interpolated model and the linear interpolation of the endpoint features, namely
% \begin{equation*}
% \Delta(\alpha) := f(\vth(\alpha)) - (1-\alpha)f(\vth_{i}) - \alpha f(\vth_{j}).
% \end{equation*}
% A small and stable $\mathcal{C}(\theta; \delta)$ indicates that the interpolation behavior remains approximately linear, thus supporting the CTL condition.

% \textbf{HVPs without Explicit Hessian Computation.} Direct computation of $\mathcal{C}(\theta; \delta) $ requires the Hessian matrix $H(\theta) = \nabla^2 f(\theta(t))$,
% which is intractable in practice due to the extremely high dimensionality of deep neural network parameter. To overcome this challenge, we estimate $\mathcal{C}(\theta; \delta)$ 
% efficiently using Hessian-vector products (HVPs) without explicitly constructing the Hessian. Fellowing Pearlmutter~\cite{pearlmutter1994fast}, a Hessian--vector 
% product $\langle\nabla^{2}f(\theta), v\rangle$ can be computed efficiently by observing that it corresponds to the directional derivative of the gradient along 
% direction $v$:
% \begin{equation}
% \nabla^{2} f(\theta)\, v
% =
% \lim_{\epsilon \to 0}
% \frac{1}{\epsilon}
% \Big[
% \nabla f(\theta + \epsilon v) - \nabla f(\theta)
% \Big]
% =
% \nabla_{\theta}
% \big(
% \langle \nabla f(\theta),\, v \rangle
% \big).
% \end{equation}
% This identity enables efficient computation of HVPs via automatic differentiation at the cost of a small constant factor over gradient computation, without 
% ever constructing the Hessian explicitly.

% After computing the Hessian-vector product $H_\theta \delta$, the deviation measure is obtained by evaluating the corresponding quadratic form:
% \begin{equation}
% \mathcal{C}(\theta; \delta) = \langle \delta, H_\theta \delta \rangle.
% \end{equation}

% \textbf{Curvature Evaluation Algorithm.} In practice, we perform curvature analysis along the parameter interpolation path from the backdoored merged model $\theta_m$ 
% to the anti-backdoor model $\theta_{k+1}$ using the adversarial dataset $\mathcal{D}_{\mathrm{adv}}$ associated with the anti-backdoor task. The overall procedure 
% is summarized in Algorithm~\ref{alg:curvature_evaluation}.
% \begin{algorithm*}[!h]
% \caption{Curvature Evaluation via Hessian--Vector Products (HVPs)}
% \label{alg:curvature_evaluation}
% \begin{algorithmic}[1]
% \STATE {\bfseries Input:} 
% Backdoored merged model $\theta_m$; 
% Anti-backdoor model $\theta_{k+1}$; 
% Number of mini-batches $N$; 
% Adversarial dataset $\mathcal{D}_{\mathrm{adv}}$; 
% Finite-difference step $\epsilon$.

% \STATE {\bfseries Output:} 
% Average quadratic form $\overline{\mathcal{C}}(\theta; \delta)$ and average effective curvature $\overline{\lambda}_{\mathrm{eff}}$.

% \vspace{0.5em}
% \STATE \textbf{Initialize:}
% $\mathcal{C}_{\mathrm{sum}} \gets 0$, \quad $\lambda_{\mathrm{sum}} \gets 0$.

% \vspace{0.5em}
% \STATE \textbf{Step 1: Compute Parameter Difference}
% \STATE $\delta \gets \theta_{k+1} - \theta_m$.
% \IF{normalize direction}
%     \STATE $\delta \gets \delta / \|\delta\|$.
% \ENDIF

% \vspace{0.5em}
% \FOR{$b = 1$ \textbf{to} $N$}
%     \STATE Sample mini-batch $\mathcal{B}_b = \{(x_i', y_i)\}$ from $\mathcal{D}_{\mathrm{adv}}$.

%     \vspace{0.3em}
%     \STATE \textbf{Step 2: Gradient at Base Parameters}
%     \STATE Compute loss $\mathcal{L}(\theta_{k+1}, \mathcal{B}_b)$.
%     \STATE Compute gradient $g_0 \gets \nabla_\theta \mathcal{L}(\theta_{k+1})$.

%     \vspace{0.3em}
%     \STATE \textbf{Step 3: Gradient at Perturbed Parameters}
%     \STATE $\theta_\epsilon \gets \theta_{k+1} + \epsilon \delta$.
%     \STATE Compute loss $\mathcal{L}(\theta_\epsilon, \mathcal{B}_b)$.
%     \STATE Compute gradient $g_\epsilon \gets \nabla_\theta \mathcal{L}(\theta_\epsilon)$.

%     \vspace{0.3em}
%     \STATE \textbf{Step 4: Estimate HVP}
%     \STATE $H_\theta \delta \gets (g_\epsilon - g_0)/\epsilon$.

%     \vspace{0.3em}
%     \STATE \textbf{Step 5: Compute Curvature Metrics}
%     \STATE $\mathcal{C}_b \gets \langle \delta, H_\theta \delta \rangle$.
%     \STATE $\lambda_b \gets \mathcal{C}_b / \|\delta\|^2$.

%     \STATE $\mathcal{C}_{\mathrm{sum}} \gets \mathcal{C}_{\mathrm{sum}} + \mathcal{C}_b$.
%     \STATE $\lambda_{\mathrm{sum}} \gets \lambda_{\mathrm{sum}} + \lambda_b$.
% \ENDFOR

% \vspace{0.5em}
% \STATE \textbf{Step 6: Average over Mini-batches}
% \STATE $\overline{\mathcal{C}}(\theta; \delta) \gets \mathcal{C}_{\mathrm{sum}} / N$.
% \STATE $\overline{\lambda}_{\mathrm{eff}} \gets \lambda_{\mathrm{sum}} / N$.

% \vspace{0.5em}
% \STATE \textbf{Return} $\overline{\mathcal{C}}(\theta; \delta)$, $\overline{\lambda}_{\mathrm{eff}}$.
% \end{algorithmic}
% \end{algorithm*}


==> section/mathematics_proof/proof_lemma_1.tex <==
\begin{proof}
Let $f:\mathcal{X}\times\Theta\to\mathcal{Y}$ denote a neural network. We consider a linear interpolation path in parameter space between two models $\theta_i$ 
and $\theta_j$, and define the interpolated model as
\begin{equation}
  \vth_{\alpha} = (1-\alpha) \vth_{i} + \alpha  \vth_{j}, \alpha \in \left[ 0,1 \right].
\end{equation}
We assume that for any fixed input $x\in\mathcal{X}$, $f(x; \vth)$ is $L_f$-Lipschitz continuous with respect to the model parameters $\vth\in\Theta$, i.e.,
\begin{equation}
\label{eq:DNN_lipschitz_continuous}
 \| f(x;\vth_i) - f(x;\vth_j) \| \le L_f \|\vth_i - \vth_j\|. 
\end{equation}
In addition, we assume that the loss function $\mathcal{L}(\cdot)$ is convex and $L_L$-Lipschitz continuous with respect to the model prediction (\eg the cross-entropy loss).

By the Lipschitz continuity of $f$ in Eq.~\ref{eq:DNN_lipschitz_continuous}, the deviation between the interpolated model and each endpoint model satisfies
\begin{equation}
\label{eq:deviation_interp_endpoint_i} 
\left \| f(x;\vth_{\alpha}) - f(x;\vth_i) \right \| \le \alpha L_f \left \| \vth_{i} - \vth_{j} \right \|
\end{equation}
and
\begin{equation}
\label{eq:deviation_interp_endpoint_j}
\left \| f(x;\vth_{\alpha}) - f(x;\vth_j) \right \| \le (1-\alpha ) L_f \left \| \vth_{i} - \vth_{j} \right \|
\end{equation}

Define the deviation between the prediction of the interpolated model and the linear interpolation of endpoint predictions as
\begin{equation}
\label{eq:deviation_interpolation_prediction}
\Delta =  f(x;\vth_{\alpha}) - \left [(1-\alpha) f(x;\vth_i) + \alpha f(x;\vth_{j}) \right ]. 
\end{equation}
By applying the triangle inequality, we obtain
\begin{equation}
\begin{aligned}
\label{eq:upper_bound_interpolation_deviation_triangle_inequality}
\left \| \Delta \right \|  &= \left \| f(x;\vth_{\alpha}) - \left [(1-\alpha) f(x;\vth_i) + \alpha f(x;\vth_{j}) \right ] \right \|  \\
&= \left \| (1-\alpha) \left [ f(x;\vth_{\alpha}) - f(x;\vth_i)\right ]  + \alpha \left [ f(x;\vth_{\alpha})- f(x;\vth_j)  \right ] \right \| \\
& \le (1-\alpha) \left \| \left [ f(x;\vth_{\alpha}) -f(x;\vth_i)\right ]  \right \| + \alpha \left \| \left [ f(x;\vth_{\alpha})- f(x;\vth_j)  \right ] \right \| \\
\end{aligned}
\end{equation}
Substituting Eqs.~\ref{eq:deviation_interp_endpoint_i} and \ref{eq:deviation_interp_endpoint_j} yields
\begin{equation}
\label{eq:upper_bound_interpolation_deviation}
\left \| \Delta \right \|  \le 2\alpha (1-\alpha)L_f\left \| \vth_{i} -\vth_{j} \right \|
\end{equation}

Since the loss function  $\mathcal{L}$ is $L_{L}-Lipschitz$ continuous, the loss deviation induced by $\Delta$ is bounded as
\begin{equation}
\label{eq:upper_bound_loss_l_lipschitz}
\left \| \mathcal{L}\big(f(x;\vth_{\alpha});y\big) - \mathcal{L}\big(\alpha f(x;\vth_{i}) + (1-\alpha)f(x;\vth_{j});y\big) \right \| \le L_{L} \left \| \Delta \right \|  
\end{equation}
Moreover, by the convexity of $\mathcal{L}$, we have
\begin{equation}
\label{eq:upper_bound_loss_convexity}
\mathcal{L}\big(\alpha f(x;\vth_{i}) + (1-\alpha)f(x;\vth_{j});y\big) \le \alpha \mathcal{L}\big( f(x;\vth_{i});y \big) + (1-\alpha )\mathcal{L}\big(f(x;\vth_{j});y\big)
\end{equation}
Combining Eqs.~\ref{eq:upper_bound_interpolation_deviation} and~\ref{eq:upper_bound_loss_l_lipschitz}, we conclude that
\begin{equation}
\label{eq:upper_bound_loss}
\mathcal{L}\big( f(x;\vth_{\alpha});y \big) \le \alpha \mathcal{L}\big( f(x;\vth_{i});y \big) + (1-\alpha )\mathcal{L}\big(f(x;\vth_{j});y \big) + 2\alpha (1-\alpha)L_{L} L_f\left \| \vth_{i} -\vth_{j} \right \|
\end{equation}
which completes the proof.
\end{proof}

